Motion-guided small MAV detection in complex and non-planar scenes

In recent years, there has been a growing interest in the visual detection of micro aerial vehicles (MAVs) due to its importance in numerous applications. However, the existing methods based on either appearance or motion features encounter difficulties when the background is complex or the MAV is too small. In this paper, we propose a novel motion-guided MAV detector that can accurately identify small MAVs in complex and non-planar scenes. This detector first exploits a motion feature enhancement module to capture the motion features of small MAVs. Then it uses multi-object tracking and trajectory filtering to eliminate false positives caused by motion parallax. Finally, an appearance-based classifier and an appearance-based detector that operates on the cropped regions are used to achieve precise detection results. Our proposed method can effectively and efficiently detect extremely small MAVs from dynamic and complex backgrounds because it aggregates pixel-level motion features and eliminates false positives based on the motion and appearance features of MAVs. Experiments on the ARD-MAV dataset demonstrate that the proposed method could achieve high performance in small MAV detection under challenging conditions and outperform other state-of-the-art methods across various metrics

==> before_document.tex <==
\usepackage{graphicx}
\usepackage{subfig}
\usepackage{amsmath}
\let\proof\relax \let\endproof\relax % to avoid confliction of amsthm with the packages such as ieeeconf
\usepackage{amsthm} % definte the proof environment: block letters + italic letters
\usepackage{amssymb}
\usepackage[font=footnotesize]{caption} % set the captain font size to 8 (i.e. footnotesize)
\usepackage{subfig} % uses subfloats within a single float MUST after the package {caption}!!
\usepackage[noadjust]{cite} % alphabetize grouped citations automatically [3, 1, 2] to [1, 2, 3]
%\usepackage{color}
%\usepackage{algorithm} % options: boxed [section]
%\usepackage{algpseudocode} % for algorithm
%\usepackage{enumerate}
%\usepackage[hidelinks,colorlinks=false]{hyperref}
%\usepackage{setspace} \setstretch{1.5}
%\usepackage[left=0.75in, right=0.75in, top=0.75in, bottom=0.75in]{geometry}
%\usepackage{authblk} % for authors' affiliation \affil{xxx}
%\usepackage{arydshln} % for dashline in table or matrix
%\usepackage{subfloat}
%\usepackage{bm}
%\usepackage{tikz}
%\usetikzlibrary{calc} % for calculation functions in Tikz let, in commands in Tikz
%\usetikzlibrary{shapes} % for block diagram
%\usetikzlibrary{chains}
%\usetikzlibrary{fit}
%\usetikzlibrary{arrows}
%\usetikzlibrary{decorations.text} % text along path
%\usetikzlibrary{decorations.markings}
%\usetikzlibrary{decorations.pathmorphing} % for zigzag arrow
%\usetikzlibrary{shadows}
%\usetikzlibrary{patterns}
%\usetikzlibrary{matrix}
%\usepackage{pgfplots}
%\usepackage[europeanresistors]{circuitikz}
%\usepackage[outline]{contour} % white surround text
%\contourlength{1.5pt}
%\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{assumption}{Assumption}
\newtheorem{remark}{Remark}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{example}{Example}
\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}

\newcommand{\tr}{\mathrm{tr}}
\newcommand{\myvec}{\mathrm{vec}}
\newcommand{\Null}{\mathrm{Null}}
\newcommand{\Range}{\mathrm{Col}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\myspan}{\mathrm{span}}
\newcommand{\mydiag}{\mathrm{diag}}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\blkdiag}{\mathrm{blkdiag}}
\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\T}{\mathrm{T}}
\newcommand{\myqed}{\hfill$\blacksquare$}
\newcommand{\ep}{\varepsilon}
\newcommand{\sig}{\mathrm{sig}_a}
%\newcommand{\sigep_}[1]{\sig(\ep_{#1})}
\newcommand{\R}{\mathbb{R}}
%\newcommand{\G}{\mathcal{G}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\D}{\mathcal{D}}
\renewcommand{\L}{\mathcal{B}}
\renewcommand{\H}{\mathcal{H}}
\renewcommand{\S}{\Omega}
\newcommand{\xe}{x_{\text{e}}}
%\newcommand{\Null}[1]{\mathrm{Null}\left(#1\right)}
\newcommand{\sk}[1]{\left[#1\right]_\times} % skew symmetric operator
\newcommand{\dia}[1]{\mathrm{diag}\left(#1\right)} % block diagnal matrix
%\renewcommand{\span}[1]{\mathrm{span}\left\{#1\right\}} % ERROR when redefine \span
\newcommand{\Db}{D_{\bar{b}}}
\newcommand{\smin}{\sigma_{\min}}
\newcommand{\smax}{\sigma_{\max}}
\newcommand{\lmin}{\lambda_{\min}}
\newcommand{\lmax}{\lambda_{\max}}
\newcommand{\emax}{\ener_{\max}}
\newcommand{\emin}{\ener_{\min}}
\renewcommand{\Re}{\mathrm{Re}}
%\newcommand{\C}{\mathbb{C}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\ener}{\varepsilon}
\newcommand{\edgeN}{n_{e}}
\newcommand{\din}{{d^{\mathrm{in}}}}
\newcommand{\dout}{{d^{\mathrm{out}}}}
\graphicspath{{figures/}}

